Asymptotic Preserving Discontinuous Galerkin Methods for a Linear Boltzmann Semiconductor Model

A key property of the linear Boltzmann semiconductor model is that as the collision frequency tends to infinity, the phase space density $f = f(x,v,t)$ converges to an isotropic function $M(v)\rho(x,t)$, called the drift-diffusion limit, where $M$ is a Maxwellian and the physical density $\rho$ satisfies a second-order parabolic PDE known as the drift-diffusion equation. Numerical approximations that mirror this property are said to be asymptotic preserving. In this paper we build two discontinuous Galerkin methods to the semiconductor model: one with the standard upwinding flux and the other with a $\varepsilon$-scaled Lax-Friedrichs flux, where 1/$\varepsilon$ is the scale of the collision frequency. We show that these schemes are uniformly stable in $\varepsilon$ and are asymptotic preserving. In particular, we discuss what properties the discrete Maxwellian must satisfy in order for the schemes to converge in $\varepsilon$ to an accurate $h$-approximation of the drift diffusion limit. Discrete versions of the drift-diffusion equation and error estimates in several norms with respect to $\varepsilon$ and the spacial resolution are also included.

==> sections/higher_order_dde_stab.tex <==
We now turn to \eqref{eqn:dt_r_J_0_bound}.  Choosing $q_h=\theta\partial_t\rho_h$ and $\tau_h = -\partial_tJ_h$ in \eqref{eqn:dde_system-b1}, adding both equations together in the system, and applying the product rule gives us
\begin{align}\label{eqn:dt_r_J_0:1}
\begin{split}
    \theta\|\partial_t\rho_h\|_{L^2(\W_x)}^2 &-(\omega J_h,\partial_t J_h)_{\W_x} - \frac{\theta}{2}\partial_t\|\ljmp \rho_h\rjmp\|_{L^2(\EIx)}^2 \\
    &- \partial_t[\theta(\grad_x\rho_h,J_h)_{\W_x}-\theta\left<\ljmp\rho_h\rjmp,\lavg J_h\ravg\right>_{\EIx}]+(E\rho_h,\partial_t J_h)_{\W_x} = 0.
\end{split}
\end{align}
Note that
\begin{align}\label{eqn:dt_r_J_0:2}
    -(\omega J_h,\partial_t J_h)_{\W_x} = -\frac{1}{2}\partial_t(\omega J_h,J_h)_{\W_x} = \frac{1}{2}\partial_t(\omega J_h,J_h)_{\W_x} -\partial_t(\omega J_h,J_h)_{\W_x},
\end{align}
and
\begin{align}\label{eqn:dt_r_J_0:3}
    (E\rho_h,\partial_t J_h)_{\W_x} = \partial_t(E\rho_h,J_h)_{\W_x} - (E\partial_t\rho_h,J_h)_{\W_x} - (\partial_t E\rho_h,J_h)_{\W_x}
\end{align}
Substituting \eqref{eqn:dt_r_J_0:2} and \eqref{eqn:dt_r_J_0:3} into \eqref{eqn:dt_r_J_0:1} and collecting like terms gives us
\begin{align}\label{eqn:dt_r_J_0:4}
\begin{split}
    \theta\|\partial_t\rho_h\|_{L^2(\W_x)}^2 &+ \frac{1}{2}\partial_t(\omega J_h,J_h)_{\W_x} + \frac{\theta}{2}\partial_t\|\ljmp \rho_h\rjmp\|_{L^2(\EIx)}^2 \\ 
    &-\partial_t\left\{(\omega J_h,J_h)_{\W_x}+\theta(\grad_x\rho_h,J_h)_{\W_x}-\theta\left<\ljmp\rho_h\rjmp,\lavg J_h\ravg\right>_{\EIx}-(E\rho_h,J_h)_{\W_x}\right\} \\
    &= (E\partial_t\rho_h,J_h)_{\W_x} + (\partial_t E\rho_h,J_h)_{\W_x}.
\end{split}
\end{align}
We see that the $\partial_t\{\ldots\}$ term in \eqref{eqn:dt_r_J_0:4} is zero by setting $\tau_h=J_h$ in \eqref{eqn:dde_system-b1-2}.  Dividing \eqref{eqn:dt_r_J_0:4} by $\theta$ and applying H\"older's and Young's inequality gives us
\begin{align}\label{eqn:dt_r_J_0:5}
\begin{split}
    \|\partial_t\rho_h\|_{L^2(\W_x)}^2 &+ \frac{1}{2\theta}\partial_t(\omega J_h,J_h)_{\W_x} + \frac{1}{2}\partial_t\|\ljmp \rho_h\rjmp\|_{L^2(\EIx)}^2
    \\
    &= \frac{1}{2}\|\partial_t\rho_h \|_{L^2(\W_x)}^2 + \frac{\|E\|_{L^\infty(\W_x)}^2}{\theta^2}\|J_h\|_{L^2(\W_x)}^2 + \frac{1}{\theta}\|\partial_t E\|_{L^\infty(\W_x)}\|\rho_h\|_{L^2(\W_x)}\|J_h\|_{L^2(\W_x)}
\end{split}
\end{align}
Integrating \eqref{eqn:dt_r_J_0:5} from $t=0$ to $T$ and applying H\"older's and Young's inequality in time yields
\begin{align}\label{eqn:dt_r_J_0:5}
\begin{split}
    \frac{1}{2}\|\partial_t\rho_h\|_{L_T^2(L^2(\W_x))}^2 &+ \frac{1}{2\theta}(\omega J_h(T),J_h(T))_{\W_x} + \frac{1}{2}\|\ljmp \rho_h(T)\rjmp\|_{L^2(\EIx)}^2
    \\
    &= \frac{1}{2}(\omega J_h(0),J_h(0))_{\W_x} + \frac{1}{2}\|\ljmp \rho_{0,h}\rjmp\|_{L^2(\EIx)}^2 \\
    &\quad+ \frac{1}{\theta^2}\big(\|E\|_{L_T^{\infty}(L^\infty(\W_x))}^2+\|\partial_t E\|_{L_T^{2}(L^\infty(\W_x))}^2\big)\|J_h\|_{L_T^2(L^2(\W_x))}^2 +  \|\rho_h\|_{L_T^\infty(L^2(\W_x))}^2
\end{split}
\end{align}
